Transactional Python for Durable Machine Learning: Vision, Challenges, and Feasibility

In machine learning (ML), Python serves as a convenient abstraction for working with key libraries such as PyTorch, scikit-learn, and others. Unlike DBMS, however, Python applications may lose important data, such as trained models and extracted features, due to machine failures or human errors, leading to a waste of time and resources. Specifically, they lack four essential properties that could make ML more reliable and user-friendly -- durability, atomicity, replicability, and time-versioning (DART). This paper presents our vision of Transactional Python that provides DART without any code modifications to user programs or the Python kernel, by non-intrusively monitoring application states at the object level and determining a minimal amount of information sufficient to reconstruct a whole application. Our evaluation of a proof-of-concept implementation with public PyTorch and scikit-learn applications shows that DART can be offered with overheads ranging 1.5%--15.6%.

==> 4.recomputing.tex <==
\section{Dynamic ID Graph Expansion}
\label{sec:recompute}

\todo{Main idea: in some cases, deltas don't need to be explicitly store.
We can save storage costs by applying computations to previously stored objects.}

To be filled in


==> figures/delta.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=8cm]{figures/delta.png}
\vspace{-4mm}
\caption{Summary of methods for capturing variable delta in the capture module. \supawit{Will re-style/simplify this}} \label{fig:delta}
\end{figure}


==> figures/examples/dummy_plot.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    height=35mm,
    width=\linewidth,
]
\end{axis}
\end{tikzpicture}
\vspace{-4mm}
\caption{Dummy plot} \label{fig:dummy}
\end{figure}


==> figures/examples/ecdf.tex <==
\begin{figure*}[t]
    \pgfplotstableread{
        x f(x)
        0 1/15
        1 2/15
        2 1/5
        3 4/15
        4 1/3
        5 0
    }\ecdfSample

    \centering
    \def\subplotwidth{0.24\linewidth}
    \def\height{40mm}
    \def\hspaceGap{0.00\linewidth}
    \def\vspaceGap{-1mm}

    \begin{subfigure}[b]{\subplotwidth}
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
        discontinuous,
        clip=false,
        jump mark left,
        ymin=0,
        ymax=1,
        xmin=0,
        xmax=5,
        % every axis plot/.style={very thick},
        table/create on use/cumulative distribution/.style={
            create col/expr={\pgfmathaccuma + \thisrow{f(x)}}   
        }
    ]
        \addplot [red] table [y=cumulative distribution]{\ecdfSample};
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{PyTorch MNIST}
    \label{fig:mltrace_mnist}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{XX}
    \label{fig:mltrace_XX}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{YY}
    \label{fig:mltrace_YY}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{ZZ}
    \label{fig:mltrace_ZZ}
    \end{subfigure}
\vspace{\vspaceGap}
\caption{Delta size eCDFs when varying sampling rate on ML scripts (PyTorch, Tensorflow, PyPerf::inference, random iPython). With line on conservative system throughput} \label{fig:mltrace}
\end{figure*}


==> figures/ml_dnn.tex <==
\begin{figure}[t]
    \centering
    \def\subplotwidth{0.48\linewidth}
    \def\height{40mm}
    \def\hspaceGap{0.00\linewidth}
    \def\vspaceGap{-1mm}

    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Delta rate (B/s) eCDF}
    \label{fig:mlperf_time}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Distortion (\%) eCDF}
    \label{fig:mlperf_distortion}
    \end{subfigure}
\vspace{\vspaceGap}
\caption{DNN Training feasibility.} \label{fig:mlperf}
\end{figure}


==> figures/ml_inference.tex <==
\begin{figure}[t]
    \centering
    \def\subplotwidth{0.48\linewidth}
    \def\height{40mm}
    \def\hspaceGap{0.00\linewidth}
    \def\vspaceGap{-1mm}

    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Delta rate (B/s) eCDF}
    \label{fig:mlperf_time}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Distortion (\%) eCDF}
    \label{fig:mlperf_distortion}
    \end{subfigure}
\vspace{\vspaceGap}
\caption{MLPerf Inference feasibility.} \label{fig:mlperf}
\end{figure}


==> figures/ml_mnist_pytorch.tex <==
\begin{figure}[t]
    \centering
    \def\subplotwidth{0.48\linewidth}
    \def\height{40mm}
    \def\hspaceGap{0.00\linewidth}
    \def\vspaceGap{-1mm}

    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Delta rate (B/s) eCDF}
    \label{fig:mlperf_time}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Distortion (\%) eCDF}
    \label{fig:mlperf_distortion}
    \end{subfigure}
\vspace{\vspaceGap}
\caption{PyTorch MNIST Training feasibility.} \label{fig:mlperf}
\end{figure}


==> figures/ml_mnist_tf.tex <==
\begin{figure}[t]
    \centering
    \def\subplotwidth{0.48\linewidth}
    \def\height{40mm}
    \def\hspaceGap{0.00\linewidth}
    \def\vspaceGap{-1mm}

    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Delta rate (B/s) eCDF}
    \label{fig:mlperf_time}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        height=\height,
        width=\linewidth,
    ]
    \end{axis}
    \end{tikzpicture}
    \vspace{\vspaceGap}
    \caption{Distortion (\%) eCDF}
    \label{fig:mlperf_distortion}
    \end{subfigure}
\vspace{\vspaceGap}
\caption{Tensorflow MNIST Training feasibility.} \label{fig:mlperf}
\end{figure}


==> figures/nested.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=5cm]{figures/nested.png}
\vspace{-4mm}
\caption{Example of a variable (\texttt{list2}) which doesn't change value, but changes relation with another variable (\texttt{list1}) after executing cell 2.} \label{fig:nested}
\end{figure}


==> figures/sys_throughput.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    height=35mm,
    width=\linewidth,
]
\end{axis}
\end{tikzpicture}
\vspace{-4mm}
\caption{Summary of system component throughput numbers (how to visualize?). Highlight the bottleneck is not too slow} \label{fig:mltrace}
\end{figure}


==> figures/tab_transaction.tex <==
\begin{table}[t]
\caption{Resemblance: DBMS and Transactional Python}
\label{tab:equivalence}
\vspace{-2mm}
\centering
\footnotesize
\begin{tabular}{lll}
    \toprule
    & \textbf{Database Transaction} & \textbf{Transactional Python} \\
    \midrule
    Data & Database/table/dataset & Observable state \\
    State & Data structures & Interpreter state \\
    Program & Transaction & Statement \\
    Machine & Transactional DBMS & Interpreter + DBMS \\
    \bottomrule
\end{tabular}
\end{table}

